Learnable Strategies for Bilateral Agent Negotiation over Multiple Issues

We present a novel bilateral negotiation model that allows a self-interested agent to learn how to negotiate over multiple issues in the presence of user preference uncertainty. The model relies upon interpretable strategy templates representing the tactics the agent should employ during the negotiation and learns template parameters to maximize the average utility received over multiple negotiations, thus resulting in optimal bid acceptance and generation. Our model also uses deep reinforcement learning to evaluate threshold utility values, for those tactics that require them, thereby deriving optimal utilities for every environment state. To handle user preference uncertainty, the model relies on a stochastic search to find user model that best agrees with a given partial preference profile. Multi-objective optimization and multi-criteria decision-making methods are applied at negotiation time to generate Pareto-optimal outcomes thereby increasing the number of successful (win-win) negotiations. Rigorous experimental evaluations show that the agent employing our model outperforms the winning agents of the 10th Automated Negotiating Agents Competition (ANAC'19) in terms of individual as well as social-welfare utilities.

==> OldSection6Results.tex <==
% \vspace*{-5mm}
\section{Experimental Results}\label{results}
All the experiments have been performed using the popular GENIUS negotiation platform~\cite{lin2014genius}.
Our experiments are designed to prove the following hypotheses:

\noindent\textbf{Hypothesis A:} Our approach can 
% derive accurate 
approximate
user models under user preference uncertainty.

\noindent\textbf{Hypothesis B:} The set of estimated Pareto-optimal bids obtained using NSGA-II are close to the true Pareto-optimal solution. 

\noindent\textbf{Hypothesis C:} \textit{ANESIA} outperforms the ``teacher'' strategies (AgentGG, KakeSoba and SAGA) in known negotiation settings in terms of individual and social efficiency.

\noindent\textbf{Hypothesis D:} \textit{ANESIA} outperforms not-seen-before negotiation strategies and adapt to different negotiation settings in terms of individual and social efficiency.
\begin{table*}
    \centering
    \resizebox{.80\textwidth}{!}{
    \begin{tabular}{p{0.10\textwidth} p{0.16\textwidth}p{0.1\textwidth}
    p{0.1\textwidth}p{0.1\textwidth}
    p{0.1\textwidth}p{0.06\textwidth}}
    \hline
      Agent &
    %   $T_{\it avg} (\downarrow)$  &  
      $R_{\it avg} (\downarrow)$  &  
      $P_{\it avg} (\downarrow)$  &  
      $U_{\it soc} (\uparrow)$  &  
      $U_{\it ind}^{total} (\uparrow)$  &  
      $U_{\it ind}^s (\uparrow)$  &
      $S_{\%} (\uparrow)$ \\  
      \hline
      ANESIA & 301.64 $\pm$ 450.60 & \textbf{0.12 $\pm$ 0.36} & \textbf{1.55 $\pm$ 0.73} & 0.39 $\pm$ 0.41 & \textbf{0.92 $\pm$ 0.11} & 0.46 \\
      AgentGG & 1327.51 $\pm$ 2246.83 & 0.30 $\pm$ 0.37 & 1.10 $\pm$ 0.67 & 0.65 $\pm$ 0.39 & 0.87 $\pm$ 0.13 & 0.75 \\
      KakeSoba & 1154.83 $\pm$ 2108.11 & 0.22 $\pm$ 0.34 & 1.26 $\pm$ 0.62 & \textbf{0.71 $\pm$ 0.35} & 0.88 $\pm$ 0.12 & 0.81 \\
      SAGA & \textbf{287.34 $\pm$ 1058.52} & 0.18 $\pm$ 0.31 & 1.36 $\pm$ 0.56 & 0.58 $\pm$ 0.26 & 0.67 $\pm$ 0.14 & \textbf{0.87 }\\
         \hline
    \end{tabular}
    }
    \caption{Performance Comparison of \textit{ANESIA} with ``teacher'' strategies. Results are averaged for all the domains and profiles. See supplement for separate results for each domains.}
    \label{table:teacher}
\end{table*}
\paragraph{Performance metrics:} 
We measure the performance of each agent in terms of seven widely-adopted metrics inspired by the ANAC competition:
\begin{itemize}
    \item $U_{\it ind}^{total}$: The utility gained by an agent averaged over all the negotiations ($\uparrow$);
    \item $U_{\it ind}^s$: The utility gained by an agent averaged over all the successful negotiations ($\uparrow$);    
    % \item $U_{\it soc}$: The utility gained by both negotiating agents averaged over all negotiations ($\uparrow$);
    \item $U_{\it soc}$: The utility gained by both negotiating agents averaged over all successful negotiations ($\uparrow$);
    \item $P_{\it avg}$: Average minimal distance of agreements from the Pareto Frontier ($\downarrow$).
    \item $R_{\it avg}$: Average number of rounds before reaching the agreement ($\downarrow$);
    % \item $T_{\it avg}$: Average amount of time to reach an agreement ($\downarrow$);
    \item $S_{\%}$: Proportion of successful negotiations ($\uparrow$).
\end{itemize}
Among the aforementioned measures, the first and second measures represent \textit{individual efficiency} of the negotiation outcome, third and fourth correspond to the \textit{social efficiency} of the agreements, 
% fifth and sixth are related to the \textit{negotiation time} elapsed before reaching the agreement; 
fifth is related to the \textit{sequence of interactions} between the two parties before reaching the agreement; 
and sixth corresponds to the \textit{negotiation success rate}.

\paragraph{Experimental settings:}  \textit{ANESIA} is evaluated against the state-of-the-art strategies that participated in the ANAC'17, '18, and '19 competitions. 
These strategies are designed by different research groups independently. Each agent has no information about other agent's strategies beforehand. Details of all these strategies are available in~\cite{aydougan2018anac, jonker2020anac, aydougan2020challenges}.
We assume incomplete information about user preferences, given in the form of $B$ randomly-chosen partially-ordered bids. 
We evaluate \textit{ANESIA} on 8 negotiation domains which are different from each other in terms of size and opposition~\cite{baarslag2013evaluating} in order to ensure good negotiation characteristics and to reduce any possible bias. The size of domain refers to the number of issues, whereas opposition\footnote{The value of opposition reflects the competitiveness between parties in the domain. Strong opposition means a gain of one party is at the loss of the other, whereas, weak opposition means that both parties either lose or gain simultaneously~\cite{baarslag2013evaluating}.}
% reflects the competitiveness
% \footnote{Strong opposition is typical of competitive domains, where a gain for one party can be achieved only at a loss for the other party. Conversely, weak opposition means that both the parties achieve either losses or gains simultaneously.} 
% degree of the negotiation domain between the negotiation parties. The opposition is defined as 
refers to
the minimum distance from all the possible negotiation outcomes to the point representing complete satisfaction of both negotiation parties (1,1). 
% \np{previous para is a bit hard to parse} 
For our experiments, we choose readily-available 3 small-sized, 2 medium-sized, and 3 large-sized domains. Out of these domains, 2 are with high, 3 with medium and 3 with low opposition. Details of these domains can be found in~\cite{williams2014overview}. 
% and are readily available in GENIUS.

% \begin{table*}
%     \centering
%     \resizebox{.98\textwidth}{!}{
%     \begin{tabular}{p{0.14\textwidth} p{0.1\textwidth}p{0.1\textwidth}
%     p{0.1\textwidth}p{0.1\textwidth}
%     p{0.1\textwidth}p{0.1\textwidth} p{0.1\textwidth}}
%     \hline
%       Agent &
%       $T_{\it avg}$  &  
%       $R_{\it avg}$  &  
%       $P_{\it avg}$  &  
%       $U_{\it soc}$  &  
%       $U_{\it ind}$  &  
%       $U_{\it ind}^s$  &
%       $S_{\%}$ \\  
%       \hline
%     ANESIA & 51.88 $\pm$ 46.93 & 1393.62 $\pm$ 1263.68 & \textbf{0.05 $\pm$ 0.18} & \textbf{1.43 $\pm$ 0.34} & \textbf{0.78 $\pm$ 0.2 }& \textbf{0.87 $\pm$ 0.13} & 0.90 \\
%     AgentGP & 92.45 $\pm$ 77.84 & 393.07 $\pm$ 658.53 & 0.18 $\pm$ 0.19 & 1.07 $\pm$ 0.38 & 0.69 $\pm$ 0.17 & 0.74 $\pm$ 0.12 & 0.84 \\
%     AgentHerb & \textbf{3.03 $\pm$ 5.36} & \textbf{18.11 $\pm$ 47.78} & 0.08 $\pm$ 0.09 & 1.34 $\pm$ 0.13 & 0.5 $\pm$ 0.14 & 0.5 $\pm$ 0.14 & \textbf{1.00} \\
%     FSEGA2019 & 80.76 $\pm$ 53.5 & 2493.66 $\pm$ 3584.12 & 0.16 $\pm$ 0.14 & 1.1 $\pm$ 0.27 & 0.69 $\pm$ 0.17 & 0.74 $\pm$ 0.14 & 0.87 \\
%     Agent33 & 51.14 $\pm$ 44.51 & 2426.17 $\pm$ 3584.54 & 0.1 $\pm$ 0.11 & 1.28 $\pm$ 0.21 & 0.61 $\pm$ 0.16 & 0.62 $\pm$ 0.16 & 0.97 \\
%     Agent36 & 130.72 $\pm$ 68.53 & 4990.53 $\pm$ 4616.11 & 0.17 $\pm$ 0.19 & 1.01 $\pm$ 0.33 & 0.72 $\pm$ 0.18 & 0.79 $\pm$ 0.12 & 0.86 \\
%     Sontag & 71.88 $\pm$ 56.16 & 4185.1 $\pm$ 5946.18 & 0.13 $\pm$ 0.13 & 1.18 $\pm$ 0.25 & 0.68 $\pm$ 0.18 & 0.71 $\pm$ 0.16 & 0.93 \\
%     AgreeableAgent & 123.6 $\pm$ 64.77 & 10035.65 $\pm$ 12035.53 & 0.15 $\pm$ 0.15 & 1.09 $\pm$ 0.29 & 0.72 $\pm$ 0.18 & 0.75 $\pm$ 0.17 & 0.91 \\
%     PonpokoAgent & 109.22 $\pm$ 72.55 & 5995.89 $\pm$ 7781.6 & 0.16 $\pm$ 0.17 & 1.04 $\pm$ 0.32 & 0.73 $\pm$ 0.17 & 0.8 $\pm$ 0.11 & 0.85 \\
%     Parscat2 & 88.51 $\pm$ 62.82 & 4698.27 $\pm$ 5548.4 & 0.12 $\pm$ 0.11 & 1.16 $\pm$ 0.22 & 0.70 $\pm$ 0.16 & 0.72 $\pm$ 0.16 & 0.94\\

%         \hline
%     \end{tabular}
%     }
%     \caption{Performance of agents averaged over all the 8 domains. See supplement for the separate results for each domain.}
%     \label{table:adaptive}
% \end{table*}
% \np{text below is repeated}.
% We assume that during negotiations, each agent has no information about its opponent's preferences and has limited information about the user preferences given in the form of $B$ randomly-chosen partially ordered bids. 
% For their respective reservation price and discount factor,  we use the default values in GENIUS. 
For each configuration, each agent plays both sides of the negotiation (e.g., buyer and seller in Laptop domain) to compensate for any utility differences in the preference profiles. We call \textit{user profile} the specific agent's role along with its associated preferences. Also, we choose two different preference uncertainties (with only $5\%$ and $10\%$ of known preferences $\Omega$).
% Since there are $9$ agents, each agent negotiates against $8$ other agents in $8$ different domains, a single tournament consists of $9 \times 8/2 \times 2 \times 8 = 576$ negotiation sessions. To reduce the effect of variation in the results, each tournament is repeated $20$ times, leading to a total of $11520$ negotiation sessions for each preference profile in a domain (which makes $11520 \times 2 = 23040$ total sessions), each with a deadline of 60s (the deadline is known to both the negotiating parties in advance). 
Moreover, we set the $u_{res}$ and $d_D$ to their respective default values, whereas deadline to 60s, normalized in $[0,1]$ (known to both negotiating parties in advance). 
% Also, we choose two user profiles and two different preference uncertainties ($B\in$ \{$5\%$ of $\omega$, $10\%$ of $\omega$\}) for each domain.

Regarding the optimization algorithms, for FA (used in hypotheses A and C), we select a population size of $20$ and $200$ generations for user model estimation and learning of strategy template parameters. We also set the maximum attractiveness value to $1.0$ and absorption coefficient to $0.01$. For NSGA-II (in hypothesis B), we choose the population size of $100$, $25$ generations and mutation count of $0.1$.
% \np{see this rewrite} 
We choose these hyper-parameters so that the run-time of the algorithms do not exceed the given timeout of 10s for deciding an action at each turn, while being able to retrieve empirically good solutions. 

\subsection{Empirical Evaluation}
\subsubsection{Hypothesis A: User Modelling} 
We use two measures to determine the difference between estimated and real user models~\cite{wachowicz2019tell}:
% basic approaches of statistical multivariate analysis as defined in~\cite{wachowicz2019tell}. 
\textit{Ordinal accuracy (OA)} 
measures the proportion of bids put by $\widehat{U}$ in the correct rank order (i.e., as defined by the true user model), where a OA value of 1 implies a 100\% correct ranking. 
% verifies the whether the estimated user model preserves the rank order for all issues and its values in domain $D$ as defined by the true user model. 
% It can be defined as the ratio of the number of elements of D for which the rank order in estimated and true user models are concordant (i.e., $n^{con}$ to the number of all elements (n+1) defined in the negotiation domain D, as shown in~\eqref{eq:oa}. 
% \begin{equation}
% \label{eq:oa}
%     OA = \frac{n^{con}}{n+1}
% \end{equation}
To capture the scale of cardinal errors, \textit{Cardinal Inaccuracy (CI)} measures the differences in ratings assigned in the estimated and true user models for all the elements in domain $D$.
% It can be defined as a multi-dimensional distance formula that determines the differences between the $n$ various issue ratings and the value ratings for each issue $j$ in estimated and true user models, as shown in~\eqref{eq:ii} and~\eqref{eq:vi} respectively.
% \begin{equation}
% \label{eq:ii}
%     II = \sum_{j=1}^{n} |w_j^{true} - w_j^{est}|
% \end{equation}
% \begin{equation}
% \label{eq:vi}
%     OI_j = w_j^{true} . \sum_{k=1}^{n_j} |\bar{v}^{true}(x_k^j) - \bar{v}^{est}(x_k^j)|
% \end{equation}
% Finally, the CI index is defined as the sum of $II$ and $OI_j$ determined for each issue $j \in {1,2,\ldots, n}$, as shown in~\eqref{eq:ci}.
% \begin{equation}
%     \label{eq:ci}
%     CI = II + \sum_{j=1}^{n} OI_j
% \end{equation}
We produced results in 8 domains and two profiles (5\% and 10\% of total possible bids) which are averaged over 10 simulations as shown in Table~\ref{table:usermodel}. All the values of OA ($\uparrow$) and CI ($\downarrow$), in each domain, for both the profiles, are above 0.6 and below 0.9 respectively, which demonstrates that our agent can uncover accurate user models under uncertainty.
% even under high uncertainty, too.

% \begin{table}
%     \centering
%       \resizebox{.42\textwidth}{!}{
%     \begin{tabular}{p{0.2\textwidth}p{0.13\textwidth}p{0.18\textwidth}}
%     \hline
%       Domain & IGD (true) $(\downarrow)$ & Average IGD (est.) $(\downarrow)$ \\
%       \hline
%     Airport Site ($|\Omega| = 420$) &  0.02  & 0.03 \\
%     Camera ($|\Omega| = 3600$) &  0.02  & 0.03  \\
%     Energy ($|\Omega| = 15625$) &  0.09  & 0.10\\
%     Fitness ($|\Omega| = 3520$) &  0.06  &  0.05 \\
%     Flight ($|\Omega| = 48$) & 0.03  &  0.01\\
%     Grocery ($|\Omega| = 1600$) &   0.04  &  0.03  \\
%     Itex-Cypress ($|\Omega| = 180$) & 0.07  &  0.09  \\
%     Outfit ($|\Omega| = 128$) &  0.02 & 0.06\\
%     \hline
%     \end{tabular}
%      }
%     \caption{Evaluation of Pareto Frontier for real and estimated utility models against one agent (AgentGG), both estimated using NSGA-II}
%     \label{table:paretoIGD}
% \end{table}
\subsubsection{Hypothesis B: Pareto-Optimal Bids} 
% To compare the distribution of Pareto front found by the NSGA-II (using estimated user and opponent models) and the true Pareto front (using real user and opponent models), we use a popular metric called Inverted Generational Distance (IGD)~\cite{cheng2012performance}.  IGD is used to measure the extent of convergence to a known set of Pareto optimal solutions. For the evaluation using estimated user and opponent models, we compute the IGD averaged over all the Pareto Frontiers generated during the negotiation against AgentGG for 5 different simulations for both the preference profiles ($|B| = 5\%$ of $\omega$ and $|B| = 10\%$ of $\omega$) in each domain.
We used a popular metric called  Inverted Generational Distance (IGD)~\cite{cheng2012performance} to compare the Pareto fronts found by the NSGA-II and the ground truth (found via brute force).
% and is defined as: 
% \begin{equation}
%     \label{eq:igd}
%     IGD(P_{true}, P_{est}) = \sum_{v \in P_{true}} \frac{d(v, P_{est})}{|P_{true}|}
% \end{equation}
% In~\eqref{eq:igd}, $P_{true}$ is a set of Pareto optimal bids in true Pareto Frontier, $P_{est}$ is a set of approximation of optimal bids in true Pareto Frontier, $d(v,P_{est})$ is the minimum Euclidean distance between $v$ and all the points in set $P_{est}$; and $|P_{true}|$ is the cardinality of set $P_{true}$.
Small IGD values suggest good convergence of solutions to the Pareto Front and their good distribution over the entire Pareto Front. 
% Table~\ref{table:paretoIGD} demonstrates the potential of NSGA-II for generating the Pareto-optimal bids as well as the closeness of estimated utility models to the true utility models.
Table~\ref{table:paretoIGD} demonstrates the potential of NSGA-II\footnote{Population size $=$ $0.02\times|\Omega|$; Number of generations $=$ 2.} for generating the Pareto-optimal bids as well as the closeness of true utility models. 
\begin{table*}[h]
    \centering
    \resizebox{.80\textwidth}{!}{
    \begin{tabular}{p{0.16\textwidth} p{0.16\textwidth}p{0.1\textwidth}
    p{0.1\textwidth}p{0.1\textwidth}
    p{0.1\textwidth}p{0.1\textwidth} p{0.1\textwidth}}
     \multicolumn{7}{c}{(A) Performance Analysis of fully-fledged ANESIA}\\
    \hline
      Agent &
    %   $T_{\it avg} (\downarrow)$  &  
      $R_{\it avg} (\downarrow)$  &  
      $P_{\it avg} (\downarrow)$  &  
      $U_{\it soc} (\uparrow)$  &  
      $U_{\it ind}^{total} (\uparrow)$  &  
      $U_{\it ind}^s (\uparrow)$  &
      $S_{\%} (\uparrow)$ \\  
      \hline

    % ANESIA & 54.32 $\pm$ 23.4 & 626.24 $\pm$ 432.45 & 0.17 $\pm$ 0.29 & \textbf{1.51 $\pm$ 0.47} & 0.66 $\pm$ 0.25 & \textbf{0.95 $\pm$ 0.06} & 0.51 \\
    %  \hline
    % \multicolumn{8}{c}{Below agents are provided with uncertain user
    % preferences, but no learning is allowed}\\
    %  \hline
    % AgentGP & 44.64 $\pm$ 31.52 & 1366.95 $\pm$ 1378.19 & 0.3 $\pm$ 0.29 & 0.82 $\pm$ 0.58 & 0.66 $\pm$ 0.25 & 0.88 $\pm$ 0.09 & 0.58 \\
    % FSEGA2019 & 47.84 $\pm$ 26.04 & 1801.96 $\pm$ 1754.91 & 0.12 $\pm$ 0.19 & 1.15 $\pm$ 0.37 & 0.74 $\pm$ 0.18 & 0.82 $\pm$ 0.11 & 0.83 \\
    %  \hline
    % \multicolumn{8}{c}{Below agents are allowed to learn from its previous negotiations, but real user preferences are given}\\
    % \hline
    % AgentHerb & \textbf{3.36 $\pm$ 5.72} &\textbf{32.3 $\pm$ 50.53} & \textbf{0.01 $\pm$ 0.03 }& 1.41 $\pm$ 0.1 & 0.45 $\pm$ 0.13 & 0.45 $\pm$ 0.13 & \textbf{1.00} \\
    % Agent33 & 36.62 $\pm$ 25.11 & 4044.47 $\pm$ 4095.57 & 0.07 $\pm$ 0.16 & 1.31 $\pm$ 0.32 & 0.62 $\pm$ 0.15 & 0.64 $\pm$ 0.14 & 0.93 \\
    % Sontag & 42.04 $\pm$ 27.1 & 5129.47 $\pm$ 5855.11 & 0.1 $\pm$ 0.18 & 1.22 $\pm$ 0.37 & 0.73 $\pm$ 0.17 & 0.79 $\pm$ 0.11 & 0.86 \\
    % AgreeableAgent & 53.37 $\pm$ 18.03 & 5003.98 $\pm$ 5216.68 & 0.11 $\pm$ 0.23 & 0.9 $\pm$ 0.4 & 0.67 $\pm$ 0.2 & 0.73 $\pm$ 0.13 & 0.73 \\
    % PonpokoAgent & 56.88 $\pm$ 31.01 & 6609.73 $\pm$ 6611.18 & 0.18 $\pm$ 0.26 & 1.01 $\pm$ 0.49 & \textbf{0.76 $\pm$ 0.22} & 0.89 $\pm$ 0.07 & 0.74 \\
    % ParsCat2 & 50.23 $\pm$ 29.18 & 4971.43 $\pm$ 4911.8 & 0.11 $\pm$ 0.22 & 1.16 $\pm$ 0.42 & 0.75 $\pm$ 0.19 & 0.81 $\pm$ 0.12 & 0.85 \\
    
    \textit{ANESIA} & \color{blue}{626.24 $\pm$ 432.45} & \color{blue}{0.17 $\pm$ 0.29} & \color{purple}{\textbf{1.51 $\pm$ 0.47}} & 0.66 $\pm$ 0.25 & \color{purple}{\textbf{0.95 $\pm$ 0.06}} & 0.51 \\
     \hline
    % \multicolumn{7}{c}{Below agents are provided with uncertain user preferences, but no learning is allowed- ANAC'19}\\
     \hline
    AgentGP $\bullet$ & 1366.95 $\pm$ 1378.19 & 0.3 $\pm$ 0.29 & 0.82 $\pm$ 0.58 & 0.66 $\pm$ 0.25 & 0.88 $\pm$ 0.09 & 0.58 \\
    FSEGA2019 $\bullet$& 1801.96 $\pm$ 1754.91 & 0.12 $\pm$ 0.19 & 1.15 $\pm$ 0.37 & 0.74 $\pm$ 0.18 & 0.82 $\pm$ 0.11 & 0.83 \\
     \hline
    % \multicolumn{7}{c}{Below agents are allowed to learn from its previous negotiations, but real user preferences are given - ANAC'17,18}\\
    \hline
    AgentHerb $\diamond$&\textbf{32.3 $\pm$ 50.53} & \textbf{0.01 $\pm$ 0.03 }& 1.41 $\pm$ 0.1 & 0.45 $\pm$ 0.13 & 0.45 $\pm$ 0.13 & \textbf{1.00} \\
    Agent33 $\diamond$ & 4044.47 $\pm$ 4095.57 & 0.07 $\pm$ 0.16 & 1.31 $\pm$ 0.32 & 0.62 $\pm$ 0.15 & 0.64 $\pm$ 0.14 & 0.93 \\
    Sontag $\diamond$ & 5129.47 $\pm$ 5855.11 & 0.1 $\pm$ 0.18 & 1.22 $\pm$ 0.37 & 0.73 $\pm$ 0.17 & 0.79 $\pm$ 0.11 & 0.86 \\
    AgreeableAgent $\diamond$& 5003.98 $\pm$ 5216.68 & 0.11 $\pm$ 0.23 & 0.9 $\pm$ 0.4 & 0.67 $\pm$ 0.2 & 0.73 $\pm$ 0.13 & 0.73 \\
    PonpokoAgent $\star$ & 6609.73 $\pm$ 6611.18 & 0.18 $\pm$ 0.26 & 1.01 $\pm$ 0.49 & \textbf{0.76 $\pm$ 0.22} & 0.89 $\pm$ 0.07 & 0.74 \\
    ParsCat2 $\star$& 4971.43 $\pm$ 4911.8 & 0.11 $\pm$ 0.22 & 1.16 $\pm$ 0.42 & 0.75 $\pm$ 0.19 & 0.81 $\pm$ 0.12 & 0.85 \\
    \hline
    \\
        \multicolumn{7}{c}{(B) Performance Analysis of ANESIA-DRL}\\

    \hline
      Agent &
    %   $T_{\it avg} (\downarrow)$  &  
      $R_{\it avg} (\downarrow)$  &  
      $P_{\it avg} (\downarrow)$  &  
      $U_{\it soc} (\uparrow)$  &  
      $U_{\it ind}^{total} (\uparrow)$  &  
      $U_{\it ind}^s (\uparrow)$  &
      $S_{\%} (\uparrow)$ \\   
      \hline
    % ANESIA & 49.93 $\pm$ 25.78 & 480.43 $\pm$ 418.81 & 0.1 $\pm$ 0.27 & \textbf{1.34 $\pm$ 0.51} & 0.65 $\pm$ 0.22 & \textbf{0.87 $\pm$ 0.14} & 0.56 \\
    %  \hline
    % \multicolumn{8}{c}{Below agents are provided with uncertain user
    % preferences, but no learning is allowed}\\
    %  \hline
    % AgentGP & 49.97 $\pm$ 30.27 & 296.58 $\pm$ 340.15 & 0.24 $\pm$ 0.25 & 0.95 $\pm$ 0.48 & 0.61 $\pm$ 0.2 & 0.69 $\pm$ 0.15 & 0.75 \\
    % FSEGA2019 & 49.19 $\pm$ 26.43 & 1488.63 $\pm$ 1924.03 & 0.22 $\pm$ 0.2 & 0.97 $\pm$ 0.39 & 0.67 $\pm$ 0.2 & 0.79 $\pm$ 0.12 & 0.77 \\
    %     \hline
    % \multicolumn{8}{c}{Below agents are allowed to learn from its previous negotiations, but real user preferences are given}\\
    % \hline
    % AgentHerb & \textbf{2.64 $\pm$ 4.78} & \textbf{38.25 $\pm$ 79.16} & \textbf{0.09 $\pm$ 0.09} & 1.33 $\pm$ 0.15 & 0.48 $\pm$ 0.16 & 0.48 $\pm$ 0.16 & \textbf{0.99} \\
    % Agent33 & 34.0 $\pm$ 24.27 & 2799.6 $\pm$ 3702.85 & 0.13 $\pm$ 0.15 & 1.22 $\pm$ 0.29 & 0.58 $\pm$ 0.15 & 0.59 $\pm$ 0.15 & 0.94 \\
    % Sontag & 41.97 $\pm$ 27.03 & 3490.01 $\pm$ 4909.81 & 0.17 $\pm$ 0.19 & 1.09 $\pm$ 0.37 & 0.69 $\pm$ 0.18 & 0.76 $\pm$ 0.13 & 0.85 \\
    % AgreeableAgent & 51.66 $\pm$ 22.82 & 3585.94 $\pm$ 4474.06 & 0.18 $\pm$ 0.21 & 0.78 $\pm$ 0.38 & 0.61 $\pm$ 0.19 & 0.68 $\pm$ 0.14 & 0.69 \\
    % PonpokoAgent & 57.04 $\pm$ 30.51 & 4470.86 $\pm$ 5482.31 & 0.25 $\pm$ 0.24 & 0.9 $\pm$ 0.45 & \textbf{0.71 $\pm$ 0.2} & 0.85 $\pm$ 0.09 & 0.72 \\
    % ParsCat2 & 48.4 $\pm$ 28.46 & 3430.55 $\pm$ 4204.93 & 0.17 $\pm$ 0.2 & 1.07 $\pm$ 0.39 & 0.69 $\pm$ 0.18 & 0.73 $\pm$ 0.16 & 0.85 \\
     ANESIA-DRL & 480.43 $\pm$ 418.81 & 0.1 $\pm$ 0.27 & \textbf{1.34 $\pm$ 0.51} & 0.65 $\pm$ 0.22 & \textbf{0.87 $\pm$ 0.14} & 0.56 \\
     \hline
    % \multicolumn{7}{c}{Below agents are provided with uncertain user preferences, but no learning is allowed- ANAC'19}\\
     \hline
    AgentGP $\bullet$ & 296.58 $\pm$ 340.15 & 0.24 $\pm$ 0.25 & 0.95 $\pm$ 0.48 & 0.61 $\pm$ 0.2 & 0.69 $\pm$ 0.15 & 0.75 \\
    FSEGA2019 $\bullet$ & 1488.63 $\pm$ 1924.03 & 0.22 $\pm$ 0.2 & 0.97 $\pm$ 0.39 & 0.67 $\pm$ 0.2 & 0.79 $\pm$ 0.12 & 0.77 \\
    \hline
    % \multicolumn{7}{c}{Below agents are allowed to learn from its previous negotiations, but real user preferences are given - ANAC'17,18}\\
    \hline
    AgentHerb $\diamond$ & \textbf{38.25 $\pm$ 79.16} & \textbf{0.09 $\pm$ 0.09} & 1.33 $\pm$ 0.15 & 0.48 $\pm$ 0.16 & 0.48 $\pm$ 0.16 & \textbf{0.99} \\
    Agent33 $\diamond$& 2799.6 $\pm$ 3702.85 & 0.13 $\pm$ 0.15 & 1.22 $\pm$ 0.29 & 0.58 $\pm$ 0.15 & 0.59 $\pm$ 0.15 & 0.94 \\
    Sontag $\diamond$ & 3490.01 $\pm$ 4909.81 & 0.17 $\pm$ 0.19 & 1.09 $\pm$ 0.37 & 0.69 $\pm$ 0.18 & 0.76 $\pm$ 0.13 & 0.85 \\
    AgreeableAgent $\diamond$ & 3585.94 $\pm$ 4474.06 & 0.18 $\pm$ 0.21 & 0.78 $\pm$ 0.38 & 0.61 $\pm$ 0.19 & 0.68 $\pm$ 0.14 & 0.69 \\
    PonpokoAgent $\star$ & 4470.86 $\pm$ 5482.31 & 0.25 $\pm$ 0.24 & 0.9 $\pm$ 0.45 & \textbf{0.71 $\pm$ 0.2} & 0.85 $\pm$ 0.09 & 0.72 \\
    ParsCat2 $\star$ & 3430.55 $\pm$ 4204.93 & 0.17 $\pm$ 0.2 & 1.07 $\pm$ 0.39 & 0.69 $\pm$ 0.18 & 0.73 $\pm$ 0.16 & 0.85 \\
        \hline
\\
    \multicolumn{7}{c}{(C) Performance analysis of Random ANESIA}\\

    \hline
      Agent &
    %   $T_{\it avg} (\downarrow)$  &  
      $R_{\it avg} (\downarrow)$  &  
      $P_{\it avg} (\downarrow)$  &  
      $U_{\it soc} (\uparrow)$  &  
     $U_{\it ind}^{total} (\uparrow)$  &  
      $U_{\it ind}^s (\uparrow)$  &
      $S_{\%} (\uparrow)$ \\  
      \hline
    % ANESIA & 35.59 $\pm$ 23.46 & 351.77 $\pm$ 343.24 & 0.17 $\pm$ 0.21 & 1.28 $\pm$ 0.43 & 0.67 $\pm$ 0.22 & 0.74 $\pm$ 0.16 & 0.80 \\
    % \hline
    % \multicolumn{8}{c}{Below agents are provided with uncertain user
    % preferences, but no learning is allowed}\\
    % \hline
    % AgentGP & 52.1 $\pm$ 28.87 & 258.12 $\pm$ 300.53 & 0.22 $\pm$ 0.24 & 1.0 $\pm$ 0.46 & 0.63 $\pm$ 0.19 & 0.70 $\pm$ 0.14 & 0.79 \\
    % FSEGA2019 & 48.06 $\pm$ 26.15 & 1002.3 $\pm$ 1349.64 & 0.2 $\pm$ 0.19 & 1.02 $\pm$ 0.35 & 0.68 $\pm$ 0.2 & 0.79 $\pm$ 0.12 & 0.81 \\
    % \hline
    % \multicolumn{8}{c}{Below agents are allowed to learn from its previous negotiations, but real user preferences are given}\\
    % \hline
    % AgentHerb & \textbf{3.64 $\pm$ 6.6} & \textbf{44.87 $\pm$ 80.16} & \textbf{0.09 $\pm$ 0.09} & \textbf{1.33 $\pm$ 0.15} & 0.48 $\pm$ 0.15 & 0.48 $\pm$ 0.15 & \textbf{0.99 }\\
    % Agent33 & 34.81 $\pm$ 23.48 & 1592.2 $\pm$ 2298.71 & 0.11 $\pm$ 0.12 & 1.26 $\pm$ 0.24 & 0.58 $\pm$ 0.15 & 0.58 $\pm$ 0.15 & 0.97 \\
    % Sontag & 41.88 $\pm$ 26.42 & 2276.96 $\pm$ 3366.2 & 0.15 $\pm$ 0.17 & 1.13 $\pm$ 0.34 & 0.70 $\pm$ 0.17 & 0.75 $\pm$ 0.13 & 0.88 \\
    % AgreeableAgent & 50.65 $\pm$ 23.08 & 2472.87 $\pm$ 3145.2 & 0.14 $\pm$ 0.17 & 0.86 $\pm$ 0.32 & 0.62 $\pm$ 0.18 & 0.67 $\pm$ 0.14 & 0.75 \\
    % PonpokoAgent & 56.39 $\pm$ 30.26 & 2825.54 $\pm$ 3745.98 & 0.22 $\pm$ 0.23 & 0.96 $\pm$ 0.41 & \textbf{0.73 $\pm$ 0.2 }& \textbf{0.84 $\pm$ 0.09} & 0.78 \\
    % ParsCat2 & 45.31 $\pm$ 26.47 & 1992.6 $\pm$ 2674.9 & 0.13 $\pm$ 0.15 & 1.07 $\pm$ 0.3 & 0.66 $\pm$ 0.17 & 0.69 $\pm$ 0.14 & 0.86 \\
     ANESIA-rand & 351.77 $\pm$ 343.24 & \color{blue}{0.17 $\pm$ 0.21} & \color{blue}{1.28 $\pm$ 0.43} & 0.67 $\pm$ 0.22 & 0.74 $\pm$ 0.16 & 0.80 \\
    \hline
    % \multicolumn{7}{c}{Below agents are provided with uncertain user
    % preferences, but no learning is allowed - ANAC'19}\\
    \hline
    AgentGP $\bullet$ & \color{blue}{258.12 $\pm$ 300.53} & 0.22 $\pm$ 0.24 & 1.0 $\pm$ 0.46 & 0.63 $\pm$ 0.19 & 0.70 $\pm$ 0.14 & 0.79 \\
    FSEGA2019 $\bullet$ & 1002.3 $\pm$ 1349.64 & 0.2 $\pm$ 0.19 & 1.02 $\pm$ 0.35 & \color{blue}{0.68 $\pm$ 0.2} & \color{blue}{0.79 $\pm$ 0.12} & \color{blue}{0.81} \\
    \hline
    % \multicolumn{7}{c}{Below agents are allowed to learn from its previous negotiations, but real user preferences are given - ANAC'17,18}\\
    \hline
    AgentHerb $\diamond$ & \color{purple}{\textbf{44.87 $\pm$ 80.16}} & \color{purple}{\textbf{0.09 $\pm$ 0.09}} & \color{purple}{\textbf{1.33 $\pm$ 0.15}} & 0.48 $\pm$ 0.15 & 0.48 $\pm$ 0.15 & \color{purple}{\textbf{0.99}}\\
    Agent33 $\diamond$ & 1592.2 $\pm$ 2298.71 & 0.11 $\pm$ 0.12 & 1.26 $\pm$ 0.24 & 0.58 $\pm$ 0.15 & 0.58 $\pm$ 0.15 & 0.97 \\
    Sontag $\diamond$ & 2276.96 $\pm$ 3366.2 & 0.15 $\pm$ 0.17 & 1.13 $\pm$ 0.34 & 0.70 $\pm$ 0.17 & 0.75 $\pm$ 0.13 & 0.88 \\
    AgreeableAgent $\diamond$  & 2472.87 $\pm$ 3145.2 & 0.14 $\pm$ 0.17 & 0.86 $\pm$ 0.32 & 0.62 $\pm$ 0.18 & 0.67 $\pm$ 0.14 & 0.75 \\
    PonpokoAgent $\star$ & 2825.54 $\pm$ 3745.98 & 0.22 $\pm$ 0.23 & 0.96 $\pm$ 0.41 & \color{purple}{\textbf{0.73 $\pm$ 0.2}}& \color{purple}{\textbf{0.84 $\pm$ 0.09}} & 0.78 \\
    ParsCat2 $\star$ & 1992.6 $\pm$ 2674.9 & 0.13 $\pm$ 0.15 & 1.07 $\pm$ 0.3 & 0.66 $\pm$ 0.17 & 0.69 $\pm$ 0.14 & 0.86 \\
        \hline
    \end{tabular}
    }
    \caption{Performance comparison of \textit{ANESIA} against other ANAC winning strategies averaged over all the 8 domains and two uncertain preference profiles. See supplement for the separate results for each domain. Note: $\bullet$ represents the ANAC'19 agents. These agents are provided with uncertain user
    preferences, and no learning is allowed. $\star$ and $\diamond$ represent the ANAC'17 and ANAC'18 agents respectively. These agents can learn from their previous negotiations, but real user preferences are given. Blue, Orange and Purple highlights the best among ANESIA and ANAC'19 agents, the best among ANESIA and ANAC'17-18 agents and the overall best respectively.}
    \label{table:hypD}
\end{table*}
\subsubsection{Hypothesis C: \textit{ANESIA} outperforms ``teacher'' strategies}
We performed a total of $1440$ negotiation sessions\footnote{$n \times (n-1)/2 \times x \times y \times z \times w = 1440$ where $n = 4$, number of agents in a tournament; $x=2$, because agents play both sides; $y=3$, number of domains; $z=20$, because each tournament is repeated 20 times; $w=2$, number of profiles in terms of B.}
% (with a deadline of 60s in each session)
to evaluate the performance of our \textit{ANESIA} agent against the three ``teacher'' strategies (AgentGG, KakeSoba and SAGA) in three domains (Laptop, Holiday, and Party) for two different profiles ($|B| = {10,20}$). These strategies were used to collect the dataset in the same domains for supervised training before the DRL process begins. Table~\ref{table:teacher} demonstrates the average results over all the domains and profiles for each agent. Clearly, our \textit{ANESIA} agent outperforms the ``teacher'' strategies in terms of $U_{\it ind}^{s}$ (i.e., individual efficiency), $U_{\it soc}$, and $P_{avg}$ (i.e., social efficiency). The results for separate domains can be found in the Appendix.

\subsubsection{Hypothesis D: Adaptive Behaviour of \textit{ANESIA} agent}
We further evaluate the performance of \textit{ANESIA} on agents (from ANAC'17, ANAC'18 and ANAC'19) unseen during training. 
% , we used a realistic set of opponent agents which had participated in ANAC'17, ANAC'18 and ANAC'19  
% For this experiment, a total of $144000$ sessions executes in GENIUS, where each agent negotiates with every other agent.
For this, we performed a total of $23040$ negotiation sessions\footnote{$n \times (n-1)/2 \times x \times y \times z \times w = 23040$ where $n = 9$; $x=2$; $y=8$; $z=20$; and $w=2$.}.
Results in Table \ref{table:hypD}(A) are averaged over all domains and profiles demonstrating that \textit{ANESIA} learns to make the optimal choice of tactics to be used at run time and outperforms other strategies\footnote{ANAC'17: Ponpoko, ParsCat2; ANAC'18: AgreeableAgent, Sontag, AgentHerb, Agent33, Agent36; ANAC'19: AgentGP, FSEGA2019. These are all the winning strategies which already exist in GENIUS and are chosen because they require minimal changes to be used for the comparison.} in terms of $U_{\it ind}^{s}$ and $U_{\it soc}$. 
\paragraph{Ablation Study 1: } We evaluate the ANESIA-DRL performance, i.e., an \textit{ANESIA} agent that does not use templates to learn optimal combinations of tactics, but uses only one acceptance tactic, given by the dynamic DRL-based threshold utility $\bar{u}_t$ (and the Boulware and Pareto-optimal tactics for bidding) for the same negotiation settings of Hypothesis D. 
% for each of 23040 sessions as that of ANESIA. 
We observe from Table \ref{table:hypD}(B) that \textit{ANESIA-DRL} outperforms the other strategies in terms of $U_{\it ind}^{s}$ and $U_{\it soc}$.
% The low successful negotiation rate as compared to other agent suggests that the set of combination of non-optimized tactics used are not very effective.

\paragraph{Ablation Study 2: } We evaluate the ANESIA-rand performance, i.e., an \textit{ANESIA} agent which starts from a random DRL policy, i.e., without any offline pre-training of the adaptive utility threshold $\bar{u}_t$, for the same negotiation settings 
of Hypothesis D. 
% for each of 23040 sessions as that of ANESIA. 
From Table \ref{table:hypD}(B), we observe in ANESIA-rand some degradation of the utility metrics compared to the fully-fledged \textit{ANESIA} and ANESIA-DRL, even though it remains equally competitive w.r.t. the ANAC'17,18 agents and outperforms the ANAC'19 agents in $P_{avg}$, $U_{\it ind}^{s}$ and $U_{soc}$. This is not unexpected because, with a poorly informed (random) target utility tactic, the agent tends to
% , at times, 
accept offers with little pay-off without negotiating for more rounds. 

From the Table \ref{table:hypD}(B) results, we conclude that the combination of both features (strategy templates and pre-training of the DRL model) are beneficial, even though these two features perform well in isolation too.  During the experiments, we observed that ANESIA becomes picky by setting the dynamic threshold utility higher and hence learns to focus on getting the maximum utility from the end agreement. This leads to low success rate as compared to other agents. 

We note that AgentHerb is the best in terms of $P_{avg}$, which is not surprising because this is one of the agents that know the true user model. This is clearly an unfair advantage over those agent, ANESIA included, who don't have this information.
% As for $P_{avg}$, we observed that AgentHerb outperforms, however, this agent belongs to the group which knows true user model, which can be seen as an unfair advantage over ANESIA. Even if this is the case, 
That said, ANESIA attains the best $P_{avg}$ among ANAC'19 agents (unaware of the true user model) and the second best lowest $P_{avg}$ among ANAC'17 and ANAC'18 agents (aware of the true user model). 
Even though they have an unfair advantage in knowing the true user model, we consider ANAC'17 and ANAC'18 agents since, like our approach, they enable learning from past negotiations. 
% allow the agents to learn from previous negotiations, as in our ANESIA approach. 

To this end, we note that \textit{ANESIA} agent uses prior negotiation data from AgentGG to pre-train the DRL-based utility threshold and adjust the selection of tactics from the templates.
The effectiveness of our approach is demonstrated by the fact that \textit{ANESIA} outperforms the same agents it was trained on (see Hypothesis C), but, crucially, so does also on domains and opponents unseen during training. 
We further stress that the obtained performance metrics are affected only in part by an adequate pre-training of the strategies: the quality of the estimated user and opponent models -- derived without any prior training data from other agents -- plays an important role too. 
The results in Tables~\ref{table:hypD} (A to C)
evidence that our agent consistently outperforms its opponents in terms of individual and social efficiency, demonstrating  that \textit{ANESIA} can learn to adapt at run-time to different negotiation settings and against different unknown opponents.
